Reconfigurable Intelligent Surface-assisted Networks: Phase Alignment Categories

The reconfigurable intelligent surface (RIS) is one of the promising technology contributing to the next generation smart radio environment. The application scenarios include massive connectivity support, signal enhancement, and security protection. One crucial difficulty of analyzing the RIS-assisted networks is that the channel performance is sensitive to the change of user receiving direction. This paper tackles the problem by categorizing the RIS illuminated space into four categories: perfect alignment, coherent alignment, random alignment, and destructive alignment. These four categories cover all the possible phase alignment conditions that a user could experience within the overall $2$ pi solid angle of RIS-illuminated space. We perform analysis for each of these categories, deriving analytical expressions for the outage probability and diversity order. Simulation results are presented to confirm the effectiveness of the proposed analytical results.

==> multi-user.tex <==

\section{Multi-user Systems Under Different MA Schemes and Synthesis Schemes}\label{syn}

With the assistance of the RIS, the channel conditions for different users can be dynamically adjusted, according to their requirements in the target data rate or service quality. In this section, we focus on discussing the feasibility of implementing of different MA protocols in the single RIS-assisted multi-user networks. More importantly, we point out that a fair comparison between TDMA and NOMA need to be done either under static RIS scenario (where the RIS only adjust the phase shift once before the transmission time block) or under dynamic RIS scenario (where the RIS can be reconfigured multiple times). The difference between the two scenarios is illustrated in Fig~\ref{rb}.

\begin{figure}[ht!]
    \begin{center}
        \includegraphics[scale=0.35]{vis_fig/rb_c.eps}
        \caption{Illustration of resource blocks for different MA schemes}
        \label{rb}
    \end{center}
\end{figure}

\subsection{Channel Model}
Consider the multi-user system where $K$ users are served by one sigle RIS. Suppose that the LoS links from the transmitter to the receivers are blocked by obstacles. The RIS is properly placed so that virtual-LoS links exist between the transmitter and the user. For convenience, we use $H(k,\bm{\theta})$ to denote the overall channel for user $k$ under the phase configuration of $\bm{\Theta}=diag(\bm{\theta})$, i.e. $H(k,\bm{\theta})=PL(k)\bm{h}^T\bm{\Theta} \bm{g_k}$.

\subsection{Static RIS Scenario}
In the static RIS scenario, once the RIS is configured according to the users locations and CSIs, it stay in the same configuration during a full transmission block. As a result, the channels to be considered in the system are $H(1,\bm{\theta_0})$,$H(2,\bm{\theta_0})$,$\cdots$, $H(K,\bm{\theta_0})$\footnote{Note that the channels are subject to a certain carrier frequency $f_0$. For different carrier frequencies, the channel of the same user under the same RIS configuration $\bm{\theta_0}$ may have significant changes}.
\subsubsection{NOMA}
As illustrated in Fig.~\ref{rb}(b), the signal of multiple users are superposed in power domain with constant power allocation throughout one transmission time block. Thus, the baseband received signal at the $k$-th user can be written as:
\begin{equation}
y_k =H(k,\bm{\theta_0})\sum_{k=1}^K\sqrt{a_k P_{rad}}\cdot x_k +n_l.
\end{equation}
Without loss of generality, we assume that $H(1,\bm{\theta_0})>H(2,\bm{\theta_0})>\cdots>H(K,\bm{\theta_0})$. If the required data rate for user $k$ is $r^*_k$, the minimum power allocated to this user should be:
\begin{equation}
    P^*_k = (2^{r^*_k}-1)(\frac{\sigma^2}{|H(k,\bm{\theta_0})|^2}+\sum_{i<k}P^*_i).
\end{equation}

From the perspective of the system, the overall multi-user network will declare an outage if the total radiated power is less than the required minimum power:
\begin{equation}\label{out_noma_sys}
P_{rad}<\sum_{k=1}^{K}P^*_k.
\end{equation}

From the perspective of a particular user, once the power allocation ($a_1$,$a_1$,$\cdots$,$a_K$) is determined, where $a_k=P_k/P_{rad}$, closed-form expression for the outage probability for user $k$ can be further determined according to the phase alignment condition of the corresponding channel $H(k,\bm{\theta_0})$. Specifically, user $k$ will declare an outage if the message of user $i$ with $i>k$ cannot be decoded under the corresponding target rate. The actual rate for user $k$ to decode the message of user $l$ ($l\geq k$ guaranteed) is:
\begin{equation}
    r_{k,l}(a_1,\cdots a_K,\bm{\theta_0})=\log_2(1+\frac{P_l}{(\frac{\sigma}{|H(k,\bm{\theta_0})|})^2+\sum_{i<l}P_i}).
\end{equation}
\begin{equation}\label{out_static_noma_0}
    P^{k}_{out}(a_1,\cdots a_K,\bm{\theta_0})=Pr\{r_{k,l}<r^*_l \}, \ \forall l\geq k.
\end{equation}
We can rewrite \eqref{out_static_noma_0} in terms of the user channel. We denote $\tau_i=2^{r^*_i}-1$, $\mu_i = \tau_i/(a_i-\tau_i\sum_{l<i}a_l)$, and $\mu^{max}_i=\max\{\mu_i,\mu_{i+1},\cdots,\mu_{K}\}$. The outage probability for user $k$ can be then expressed as:
\begin{equation}
    P^{k}_{out}(P^*_1,\cdots P^*_K,\bm{\theta_0})=Pr\{|H(k,\bm{\theta_0})|^2 < \mu^{max}_k\}.
\end{equation}
According to Section~\ref{asymp}, for users located at the target direction, the outage probability has the asymptotic expression as:
\begin{equation}\label{asymp_noma_static}
    P_{out}^{k} = \frac{b^{-M}\mu_k^M}{(2M)!}(\frac{\sigma^2}{P_{rad}})^M.
\end{equation}
It is clear that a diversity order of $M$ is achieved for these users. For users located at other directions and experience random phase alignment overall channels, the outage probability can be expressed as:
\begin{equation}\label{ana_noma_static}
    P_{out}^{k} = 1- exp(\frac{\mu_k\sigma^2}{M P_{rad}}).
\end{equation}
These users have diversity order of one.

\subsubsection{TDMA}
As illustrated in Fig.~\ref{rb}(a), for TDMA scheme in the static RIS scenario, different users are served in different time slots. However, the RIS configuration remains the same in these time slots. If the required data rate for user $k$ is $r^*_k$, the minimum power required in the corresponding TDMA time slot should be:
\begin{equation}
    P^{TDMA}_k = (2^{Kr^*_k}-1)(\frac{\sigma^2}{|H(k,\bm{\theta_0})|^2}).
\end{equation}
From the perspective of the system, the system will declare an outage if:
\begin{equation}\label{out_tdma}
    P_{rad}< \frac{1}{K}\sum_{k=1}^K P^{TDMA}_k.
\end{equation}
It has been proven in \cite{chen2017optimization} that for the scenario where the users required the same minimum data rate $r^*_k \equiv r^*$, the outage probability of TDMA in \eqref{out_tdma} is always greater or equal to the outage probability of NOMA in \eqref{out_noma_sys}. The outage probability for each user from the user perspective can be obtained in the similar way as in the analysis of NOMA users.

\subsubsection{FDMA}
Studying FDMA scheme in the RIS-assisted network has some unique challenges. For the static RIS scenario, there are also $K$ relevant channels in the system, denote as $H^{F}(1,\bm{\theta_0})$,$H^F(2,\bm{\theta_0})$,$\cdots$, $H^F(K,\bm{\theta_0})$. As shown in Fig~\ref{rb}(d), due to the fact that FDMA scheme allocate resource blocks with different carrier frequencies to different users, even under the same RIS phase shift configuration $\theta_0$, the overall channel for the FDMA user is different from the NOMA user or TDMA user. Namely, $H^F(k,\bm{\theta_0}) \neq H(k,\bm{\theta_0})$, if the carrier frequency of the FDMA user is different from the the NOMA user or TDMA user. As a result, a practical comparison between NOMA/TDMA and FDMA should not base on the assumption that the user $k$ has the same channel condition in different MA schemes. If the required data rate for user $k$ is $r^*_k$, the minimum power required in the corresponding TDMA time slot should be:
\begin{equation}
    P^{FDMA}_k = (2^{Kr^*_k}-1)(\frac{\sigma^2}{K|H(k,\bm{\theta_0})|^2}).
\end{equation}



\subsection{Dynamic RIS Scenario}
This requires the RIS to reconfigure itself more than once during the transmission block. Here, we focus on the scenario where the RIS changes its configuration in each of the $K$ time slots. Thus, there are a number of $K^2$ channels that is relevant to our discussion: $H(1,\bm{\theta_1})$,$H(2,\bm{\theta_1})$,$\cdots$,$H(K,\bm{\theta_1})$,$H(1,\bm{\theta_2})$,$H(2,\bm{\theta_2})$,$\cdots$, $H(K,\bm{\theta_2})$,$\cdots$,$H(1,\bm{\theta_K})$,$H(2,\bm{\theta_K})$,$\cdots$,$H(K,\bm{\theta_K})$.


\subsubsection{NOMA (hybrid)}
As illustrate in Fig~\ref{rb}(c), in the dynamic RIS scenario, the NOMA users are allocated with different powers in different time slots. For convience, we denote the SINR for user $k$ to decode its own message in time slot $t$ as $\gamma_k^{(t)}$. This SINR is determined by the channel ordering and power allocated to user $k$ in time slot $t$ (denoted by $P_k^{(t)}$). Suppose that the required data rate for user $k$ is $r^*_k$, the power allocated to user $k$ in each time slot should satisfy:
\begin{equation}
\sum_{t=1}^K r_k(t) = \sum_{t=1}^K \log_2(1+\gamma_k^{(t)}) \geq r^*_k,
\end{equation}
where $r_k(t)$ is the rate of user $k$ in time slot $t$. Generally speaking, this rate can be set to different optimized values in different time slot. In order to compare with TDMA, we consider the scenario where the rate is set as $r_k(t) \equiv r^*_k/K$. Thus, the minimum required power allocated to user $k$ in time slot $t$ can be expressed as:
\begin{equation}
    P_k^{(t)} = (2^{r^*_k}-1)(\frac{\sigma^2}{|H(k,\bm{\theta_t})|^2}+\sum_{i<k}P^{(t)}_i).
\end{equation}
From the perspective of the system, the system will declare an outage if:
\begin{equation}\label{out_noma}
    P_{rad}< \sum_{t=1}^K \sum_{k=1}^K P^{(t)}_k.
\end{equation}


\subsubsection{TDMA}
For TDMA scheme in the dynamic RIS scenario, different users are served in different time slots, with different RIS configurations. If the required data rate for user $k$ is $r^*_k$, the minimum power required in the corresponding time slot  should be:
\begin{equation}
    P^{TDMA}_k = (2^{Kr^*_k}-1)(\frac{\sigma^2}{|H(k,\bm{\theta_k})|^2}).
\end{equation}
From the perspective of the system, the system will declare an outage if:
\begin{equation}\label{out_tdma_2}
    P_{rad}< \sum_{k=1}^K P^{TDMA}_k.
\end{equation}
Again, it can be proved that the mininum required power for NOMA and TDMA in the dynamic RIS scenario also satisfy:
\begin{equation}
    \sum_{k=1}^K P^{TDMA}_k \geq \sum_{t=1}^K \sum_{k=1}^K P^{(t)}_k.
\end{equation}


\begin{comment}


For LoS-dominant links $\bm{h}$ and $\bm{g_k}$, the cascaded channel through the $m$-th element takes the following form:
\begin{equation}\label{cascaded}
h_mg_{m,k} = |c_{km}|e^{2\pi ju_k\frac{d_x}{\lambda} m},
\end{equation}
where $u_k$ is related to the angle of the $k$-th receiver. After normalization, we indicate the term $exp({-2\pi ju_k\frac{d_x}{\lambda} m})$ as the exponential factor of the RIS environment. The radiation pattern function is the complex excitation coefficients of the RIS elements multiplied with the exponential factor:
\begin{equation}\label{r_patt}
F(u_k)=\sum_{m=1}^M c'_m e^{2\pi ju_k\frac{d_x}{\lambda} m}.
\end{equation}
For single RIS-assisted multiple users networks, different radiation pattern ($F(u)$) is desired. Thus, the corresponded RIS pattern which enables the desired pattern needs to be designed.
\end{comment}



\subsection{Minimum required angular distance between two users to transpose channel ordering}
One of the main challenges of serving multiple users with the assistance of a single RIS under NOMA scheme is the channel ordering problem. In the RIS-assisted networks, because the RIS does not have the ability to receive and decode signals, real-time CSI for $\bm{h}$ and $\bm{g_k}$ are hard to obtain. As a result, even for a fixed RIS phase shift configuration, channel order is constantly changing for users located at different directions and different distance w.r.t. the RIS. To address and understand this problem, we discuss under the 1-D phase scanning RIS configuration, the minimum required angular distance for two users to transpose their decoding orders.

Consider a pair of users served spontaneously by the RIS under NOMA principle. Without loss of generality, suppose the distance between the users and the RIS follows: $d_1>d_2$. The following theorem describe the minimum angular spacing required to decode the near user information first:

\begin{theorem}\label{theorem_NOMA}
In order for the RIS to transpose the decoding order for the near user and the far user, the angular spacing ($\Delta\varphi$) between the two user should satisfy:
\begin{equation}\label{spacing}
\sin(\Delta\varphi) \geq \sqrt{\frac{6}{\pi^2(M^2-1)}(\frac{\lambda_c}{d_x})^2(1-\frac{d_2^\beta}{d_1^\beta})},
\end{equation}
where $\beta$ is the pass loss parameter and $d_1,d_2$ denote the distance between the two users and the RIS. For LoS dominated links $\bm{g_k}$, it is safe to take $\beta=2$.
\begin{proof}
According to the NOMA principles, in order for the far user (user 1) to be decoded first, the channel condition should satisfy:
\begin{equation}\label{noma_con}
    PL(d_1)|\bm{h}^T\bm{\Phi} \bm{g_1}| > PL(d_2)|\bm{h}^T\bm{\Phi} \bm{g_2},
\end{equation}
where the diagonal matrix $\bm{\Phi}$ is configured according to \eqref{c_scan}. The target direction indicated by $u_0$ in \eqref{c_scan} is chosen to be the direction of the far user. Under this setting, according to \eqref{pattern_0}, we can obtain the ratio between two small-scale fading of the two users:
\begin{equation}\label{ratio_2}
    \frac{|\bm{h}^T\bm{\Phi} \bm{g_2}|}{|\bm{h}^T\bm{\Phi} \bm{g_1}|} = \frac{\sin[M\pi d_x(\sin\varphi)/\lambda_c]}{M\sin[\pi d_x(\sin\varphi)/\lambda_c]},
\end{equation}
where $\varphi$ denote the angular spacing between the two users. For small $\varphi$, we keep the first two dominate terms in the Taylor series of the RHS of \eqref{ratio_2}. Thus, \eqref{noma_con} can be expressed as:
\begin{equation}
    (\pi\frac{d_x}{\lambda_c}\sin\varphi)^2<\frac{6(PL(d_1)/PL(d_2))}{1-M^2}.
\end{equation}
Finally, using the pass loss model presented in Section~\ref{sys_m}, we can arrive at \eqref{spacing} in Theorem~\ref{theorem_NOMA}.
\end{proof}
\end{theorem}

\begin{table}[!h]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
$M$ & $d_1/d_2$ & $d_x/\lambda_c$ & $\Delta\varphi$ \\ \hline
5   & 2         & 0.5            & 16.0$^\circ$         \\ \hline
10  & 2         & 0.5            & 7.8 $^\circ$            \\ \hline
10  & 4         & 0.5            & 8.7$^\circ$             \\ \hline
10  & 2         & 0.25           & 15.8$^\circ$            \\ \hline
15  & 2         & 0.5            & 5.2$^\circ$             \\ \hline
\end{tabular}
\caption{Required angular spacing for transpose decoding order in RIS networks.}
\label{table_spacing}
\end{table}

\begin{remark}
Form Table~\ref{table_spacing}, we can observe that the required spacing quickly decreases with the increase of the number of elements ($M$). This result is consistent with Theorem~\ref{theorem_0} since as the $M$ increases, the radiated power is more concentrated within the target direction. Moreover, the distances between the users and the RIS and the elements size also have impact on the required angular spacing.
\end{remark}





\subsection{Other Synthesis Techniques (with Amplitude Control)}
Leveraging the fact that the radiation pattern of the uniform 1-D phase scanning RIS in \eqref{pattern_0} forms an orthogonal set with different $u_i=\lambda/(Md_x)\cdot i$, where $i=0,\pm 1, \pm 2,\cdots \pm (M-1)/2$ for odd $M$. As a result, if the desired radiation pattern can be written as a superposition of these $M$ orthogonal 1-D phase scanning pattern:
\begin{equation}\label{super}
F(u) = \sum_{i} \alpha_iF(u_i),
\end{equation}
then, the corresponding Woodward Synthesis pattern can be given by:
\begin{equation}\label{wood}
c'_m=\sum_i \alpha_i \cdot exp(2\pi ju_i\frac{d_x}{\lambda} m),
\end{equation}

\begin{figure}[ht!]
    \begin{center}
        \includegraphics[scale=0.6]{fig/range}
        \caption{Radiation pattern for 17-element 1-D WoodWard synthesis pattern.}
        \label{pattern_fig_1}
    \end{center}
\end{figure}

The Woodward synthesis is a proper choice for the static RIS scenario, where multiple users require similar power levels within a relatively wide angle range. As illustrated in Fig.~\ref{pattern_fig_1}, the Woodward synthesis produces a nearly constant power level within the targeted angle of $\sin\theta\in (0.3,0.6)$, indicating the 3-dB beamwidth is roughly $19.4$ degree.

\begin{remark}
It is worth pointing out that, according to \eqref{wood}, the complex excitation coefficients for the RIS elements have different magnitudes. As a result, to achieve Woodward synthesis, amplitude control at the RIS is required. As illustrated in Fig.~\ref{pattern_fig_1}, without amplitude control, a uniform synthesis method will result in a much degraded radiation pattern with stronger sidelobes.
\end{remark}


==> system_model.tex <==
Suppose the transmitter (T) and the receiver (R) both has single antenna. The RIS has a number of $M$ distinct elements, each associated with the signal response of $\tilde{a}_m=|a_m|\cdot e^{\phi_m}$. At the receiving antenna, there are $M$ signal paths. Consider the in-the-air add up of these $M$ diversity branch, the total signal can be expressed as:
\begin{align}\label{signal_total}
\begin{split}
r(t)= [\sum_{m=1}^M |g_m|\cos(\psi_m+\phi_m)]\cos\omega_c t\\
+[\sum_{m=1}^M |g_m|\sin(\psi_m+\phi_m)]\sin\omega_c t.
\end{split}
\end{align}
where $
|g_m| = \sqrt{(g^c_m)^2+(g^s_m)^2}
$,$
\psi_m=\arctan(\frac{g^s_m}{g^c_m})
$ and $g^c_m$ and $g^c_m$ are the inphase and quadrature components of the $m$-th received envelope. 

In prior works, the received signal are usually expressed as the transmitted signal multiplies with the channel gains and the phase shifts. Typically, the noiseless received signal is characterized as:
\begin{equation}\label{signal_prior}
r(t) = (\sum_{m=1}^M h^{T,I}_mh^{I,R}_m e^{\phi_m})\cdot s(t),
\end{equation}
where $h^{T,I}_m$ denote the complex channel between the transmitter and the $m$-th RIS element, and $h^{I,R}_m$ denote the complex channel between the $m$-th RIS element and the receiver. 

We can unite the two expressions in \eqref{signal_total} and \eqref{signal_prior} if we use define the complex envelope of $g_m$ as:
\begin{equation}\label{com_env}
\tilde{g}_m= g^c_m + jg^s_m = |g_m|e^{j\psi_m}.
\end{equation}
Then, in \eqref{signal_prior}, we replace $h^{T,I}_mh^{I,R}_m$ with $|g_m|e^{j\psi_m}$ and use an unmodulated signal: $s(t)=e^{\omega_ct}$, we have:
\begin{equation}\label{com_version}
\tilde{r}(t)=(\sum_{m=1}^M |g_m|e^{j(\psi_m+\phi_m)})\cdot e^{\omega_c t}.
\end{equation}
Thus, the expression of the complex received signal is united with the quadrature form in \eqref{signal_total}. Finally, $h_m$ in \eqref{superposition} can be defined as: $|h_m|=|g_m|$ and $\theta_m=\psi_m+\phi_m$. In fading environments, the $m$-th diversity branch can be expressed as:
\begin{equation}
    h_m = PL(m)\bar{h_m},
\end{equation}
where $\bar{h_m}$ is the normalized small-scale distribution of the channel, $PL(m) = \frac{p^2_xp^2_y}{16\pi^2d^2_1d^2_2}D^2G_tG_r$, $D(\theta,\varphi)$ is the pattern directivity of the RIS element, $G_r$ and $G_t$ are the gain of the receiving and transmitting antenna, $p_x$ and $p_y$ are the geometrical size of each element.

\subsection{Array Gain and Diversity Gain of the RIS-assited Networks}
In strong fading environment, diversity-combining is a powerful technique to take advantage of the lack of correlations in the rapid fluctuations (multipath fading) between different signal paths. Under proper combining schemes, the overall received signal exhibits a more desirable power distribution with less fading. In this paper, we regard the RIS as a realization to achieve spacial diversity (producing multiple diversity branches). However, compared with spacial diversity achieved by deploying multiple transmit or receive antennas, the characteristic of the RIS is unique in the following ways:
\begin{itemize}
\item Comparing with receiver diversity, the in-the-air add up of the different signal paths produced by the RIS avoids the addition of noise in each receiving branch.
\item Comparing with transmitter diversity, the constraint of a constant transmitting power is replaced by the energy conservation law for the reflection incidents at the RIS.
\item Because the spacing of the RIS element is typically smaller than a wavelength, the correlation between the signal of different diversity branches need to be taken account. Strong correlation will cause degradation in the diversity performance. This degradation is ignored in our analysis.
\end{itemize}
The combined received SNR at the receiver is:
\begin{align}\label{snr_con}
\gamma_{\Sigma}&=\frac{P_r}{N_0B}=M^2\cdot\frac{PL(m)E_s}{N_0BT_s},
\end{align}
where $N_0/2$ is the power spectral density of $n_0$, $2B$ is the bandwidth of the transmitted signal $s(t)$, $E_s$ is the energy per symbol, and $T_s$ is the symbol time. This result shows that even in the absence of multipath fading, the presence of the RIS achieved an $M^2$-fold increase in SNR due to the co-phase combining of different branches. This gain in SNR is an analogy to the \textbf{\textit{array gain}}. The \textbf{\textit{diversity gain}} due to the RIS is further presented in the analysis of the diversity order in Section~\ref{asymp}.

\begin{comment}


\subsection{Path Loss Model}

We analyse the path loss by studying the specular component of $h^{T,I}_m$ and $h^{I,R}_m$. Assuming perfect CSI at the RIS, the optimal phase shift of each element should be chosen as: $\phi_m = -\phi^\alpha_m-\phi^\beta_m$, for $m=1,2,...,M$. We further assume that the RIS elements perform no amplitude change, indicating $|a_m|=1$. As a result, the received signal can be reduced to:
\begin{equation}\label{signal_re}
r = (\sum_{m=1}^M \alpha_m\beta_m)\cdot s +n.
\end{equation}
Next, the path loss of the T-RIS links ($\alpha_m$) and RIS-R links ($\beta_m$) is investigated. Consider the transmitting antenna at T has a power gain of $G_t$ with transmitting power of $P_{rad}$. At the RIS, the time-averaged Poynting flux is:
\begin{equation}\label{flux}
\langle u\rangle=G_t\frac{P_{rad}}{4\pi \bar{d_1}^2},
\end{equation}
where $\bar{d_1}$ is the average distance from T to each RIS elements. Note that $\langle u\rangle$ has a unit of W/m$^2$. The incident electromagnetic wave (EM wave) on the RIS can be characterized by its electric field, whose amplitude is related to the Poynting flux as:
\begin{equation}\label{efield}
|E_{in}|=\sqrt{\frac{2\langle u\rangle}{\epsilon_0c}},
\end{equation}
where $\epsilon_0$ is the free space permittivity and $c$ is the speed of light. Suppose the RIS elements are rectangular with size $p_x \times p_y$, then, in the far-field\footnote{Further discussion about the definition of the far-field, as well as its boundary with the near-field can be found in the "survey paper"}, the received electric field contributed by the $m$-th element is:
\begin{equation}\label{e_r}
|E^{(m)}_r|=\frac{p_xp_y}{\lambda d_2}D(\theta_{out},\phi_{out})|E_{in}|,
\end{equation}
where $D(\theta,\varphi)$ is the pattern directivity of the RIS element and $\lambda$ is the signal wavelength. 

In strong fading environment, diversity-combining is a powerful technique to take advantage of the lack of correlations in the rapid fluctuations (multipath fading) between different signal paths. Under proper combining schemes, the overall received signal exhibits a more desirable power distribution with less fading. In this paper, we regard the RIS as a realization to achieve spacial diversity (producing multiple diversity branches). However, compared with spacial diversity achieved by deploying multiple transmit or receive antennas, the performance of the RIS is unique in the following ways:
\begin{itemize}
\item Comparing with receiver diversity, the in-the-air add up of the different signal paths produced by the RIS avoids the addition of noise in each receiving branch.
\item Comparing with transmitter diversity, the constraint of a constant transmitting power is replaced by the energy conservation law for the reflection incidents at the RIS.
\item Because the spacing of the RIS element is typically smaller than a wavelength, the correlation between the signal of different diversity branches need to be taken account. Strong correlation will cause significant degradation in the diversity performance. This degradation is ignored in our analysis.
\end{itemize}
We define a concept similar to the average SNR for each branch, in the analysis of receiver diversity. Suppose we consider each T-($m$-th element)-R link as a receiving branch. Although these ``receiving branches" are added up ``in the air" before received by the signal receiving antenna, it is still reasonable to consider the power gain for each branch. In reality, this can be achieved by ``turning off" all other elements (setting their amplitudes $|a_m|$ as zero). Thus, we write down the time-averaged Poynting flux at the receiver induced by a single branch:
\begin{equation}\label{flux_r}
\langle u^{(m)}_r\rangle = (\frac{p_xp_y}{\lambda d_2})^2D^2G_t\frac{P_{rad}}{4\pi d_1^2}.
\end{equation}
Suppose the receiving antenna has a gain of $G_r$, then the received power for each branch is:
\begin{align}\label{pr_each}
\begin{split}
P^{(m)}_r
&=\langle u^{(m)}_r\rangle \frac{G_r\lambda^2}{4\pi} \\
&=\frac{p^2_xp^2_y}{16\pi^2d^2_1d^2_2}D^2G_tG_rP_{rad}.
\end{split}
\end{align}
For convenience, we denote the term $\frac{p^2_xp^2_y}{16\pi^2d^2_1d^2_2}D^2G_tG_r=P^{(m)}_r/P_{rad}$ as $PL^{(m)}$.
Relating with \eqref{signal_re}, it can be inferred that:
\begin{equation}\label{joint}
\alpha_m\beta_m = \sqrt{PL^{(m)}}.
\end{equation}
Finally, the SNR for each branch can be defined as:
\begin{align}\label{snr_b}
\gamma_m=\frac{P^{(m)}_r}{N_0B}=\frac{\alpha^2_m\beta^2_mE_s}{N_0BT_s},
\end{align}
where $N_0/2$ is the power spectral density of $n_0$, $2B$ is the bandwidth of the transmitted signal $s(t)$, $E_s$ is the energy per symbol, and $T_s$ is the symbol time. At the same time the combined received SNR at the receiver is:
\begin{align}\label{snr_con}
\gamma_{\Sigma}&=\frac{P_r}{N_0B}=M^2\cdot\frac{\alpha^2_m\beta^2_mE_s}{N_0BT_s}.
\end{align}
This result shows that even in the absence of multipath fading, the presence of the RIS achieved an $M^2$-fold increase in SNR due to the co-phase combining of different branches. This gain in SNR is an analogy to the \textbf{\textit{array gain}}, defined as:
\begin{equation}\label{array_gain}
A_g = \frac{\gamma_\Sigma}{\bar{\gamma}_m}.
\end{equation}


In the following discussion, we also investigate the \textbf{\textit{diversity gain}} in the multipath fading environment. However, before the discussion, it is crucial to explicitly derive expression for $\alpha_m$ and $\beta_m$, instead of their multiplication. The T-RIS links ($h^{T,I}_m$) need to be further defined. The reason is that there are no actual receiving antennas at the location of the RIS and the signal is not received or decode there. The signal is simply reflected base on physical principles, similar to the reflection of the signal with the environment in multipath links. 

We take the approach to clarify this obscurity by defining the equivalent radiating power for each RIS element. The choice of $P^{(m)}_{eff}$ should ensure that the R receives the same signal power, while removing T:
\begin{equation}\label{equiv1}
\frac{D^2}{4\pi d^2_2}P^{(m)}_{eff}= \langle u^{(m)}_r\rangle.
\end{equation}
Using the result in \eqref{flux_r}, we have:
\begin{equation}\label{equiv2}
P^{(m)}_{eff}=\frac{p^2_xp^2_y}{\lambda^2d^2_1}G_tP_{rad}.
\end{equation}
The RIS-R links ($h_m$) and their amplitudes $\beta_m$ can be defined as:
\begin{equation}
\beta_m = \sqrt{\frac{P^{(m)}_r}{P^{(m)}_{eff}}}=\frac{D\lambda}{4\pi d_2}\sqrt{G_r}.
\end{equation}
As a result, using \eqref{joint}, we have:
\begin{equation}\label{alpha}
\alpha_m = \sqrt{PL^{(m)}}/\beta_m=\frac{p_xp_y}{d_1\lambda}\sqrt{G_t}.
\end{equation}
Finally, we arrive at the path loss expression for the $m$-th T-RIS channel ($\alpha_m$) and RIS-R channel ($\beta_m$).

\end{comment}
